Edge-free but Structure-aware: Prototype-Guided Knowledge Distillation from GNNs to MLPs

Distilling high-accuracy Graph Neural Networks (GNNs) to low-latency multilayer perceptions (MLPs) on graph tasks has become a hot research topic. However, conventional MLP learning relies almost exclusively on graph nodes and fails to effectively capture the graph structural information. Previous methods address this issue by processing graph edges into extra inputs for MLPs, but such graph structures may be unavailable for various scenarios. To this end, we propose Prototype-Guided Knowledge Distillation (PGKD), which does not require graph edges (edge-free setting) yet learns structure-aware MLPs. Our insight is to distill graph structural information from GNNs. Specifically, we first employ the class prototypes to analyze the impact of graph structures on GNN teachers, and then design two losses to distill such information from GNNs to MLPs. Experimental results on popular graph benchmarks demonstrate the effectiveness and robustness of the proposed PGKD.

==> tables/abalation_merge.tex <==
\begin{table}[!th]
\centering%
\renewcommand\arraystretch{1.4}
\begin{minipage}[b]{0.48\textwidth}
\centering%
\caption{The ablation accuracy~(\%) on \textbf{Citeseer} dataset for several GNN teachers under \textit{inductive} setting.
We report the results for five runs.}
\label{tab:abaltion}
\resizebox{\textwidth}{!}
{%
\begin{tabular}{lcccc}
\hline
\textbf{Model} & \textbf{SAGE} & \textbf{GAT} & \textbf{GCN} & \textbf{APPNP} \\ \hline
GNN            & 69.89$\pm$2.83    & 71.69$\pm$2.90    & 70.83$\pm$3.12   & 72.93$\pm$2.11     \\
GLNN           & 69.34$\pm$2.10    & 69.12$\pm$3.83   & 69.01$\pm$2.92   & 69.23$\pm$1.74     \\ \hline
PGKD           & 69.94$\pm$2.03    & 69.89$\pm$4.51   & 70.00$\pm$2.00   & 69.78$\pm$1.59     \\
\quad -$\mathcal{L}_{intra}$           & 69.01$\pm$1.76    & 68.51$\pm$5.03   & 69.28$\pm$2.28   & 68.62$\pm$1.77     \\
\quad -$\mathcal{L}_{inter}$           & 68.62$\pm$2.87    & 69.17$\pm$3.62   & 69.12$\pm$1.98   & 68.23$\pm$2.01     \\ \hline
\end{tabular}
}
\end{minipage}%
\hspace{3mm}%
\begin{minipage}[b]{0.48\textwidth}
\centering%
\caption{The ablation results~(\%) on \textbf{Cora} dataset for several GNN teachers under \textit{transductive} setting.
We report the results for five runs.}
\label{tab:abaltion2}
\resizebox{\textwidth}{!}
{%
\begin{tabular}{lcccc}
\hline
\textbf{Model} & \textbf{SAGE} & \textbf{GAT} & \textbf{GCN} & \textbf{APPNP} \\ \hline
GNN            & 81.11$\pm$2.05    & 81.81$\pm$1.28    & 82.24$\pm$0.59   & 83.26$\pm$0.87     \\
GLNN           & 80.22$\pm$1.81    & 79.92$\pm$1.00   & 81.43$\pm$0.18   & 79.40$\pm$1.34     \\ \hline
PGKD           & 82.15$\pm$0.19    & 81.65$\pm$1.47   & 82.39$\pm$0.64   & 82.59$\pm$1.11     \\
\quad -$\mathcal{L}_{intra}$           & 80.83$\pm$1.26    & 80.21$\pm$1.10   & 81.12$\pm$0.92   & 79.55$\pm$1.04     \\
\quad -$\mathcal{L}_{inter}$           & 81.17$\pm$1.62    & 81.98$\pm$1.04   & 81.91$\pm$0.54   & 82.79$\pm$0.86     \\ \hline
\end{tabular}
}
\end{minipage}

\end{table}


==> tables/intra_inter.tex <==
\begin{table}[!th]
\centering%
\renewcommand\arraystretch{1.4}
\begin{minipage}[b]{0.48\textwidth}
\centering%
\caption{
Average L2 distance for the features of connected nodes on different datasets.
% We adapt SAGE for GNN teacher.
% GLNN learns MLP by vanilla logit-base KD.
}
\label{tab:intr_dis}
\resizebox{\textwidth}{!}
{%
\begin{tabular}{lcccc}
\hline
\textbf{Dataset}    & \textbf{Input}   & \textbf{GNN}  & \textbf{GLNN} & \textbf{PGKD} \\ \hline
Cora       & 4.40  & 1.95 & 3.02 & 2.47 \\
Citeseer   & 5.66  & 1.40 & 3.10 & 0.82 \\
A-computer & 17.63 & 2.35 & 7.14 & 4.76 \\ \hline
\end{tabular}
}
\end{minipage}%
\hspace{3mm}%
\begin{minipage}[b]{0.48\textwidth}
\centering%
\caption{
Spearman correlation $\rho$ between class distances and inter-class edges quantity.
$\rho \to -1$ indicates more negatively correlated for two variables.
}
\label{tab:inter}
\resizebox{\textwidth}{!}
{%
\begin{tabular}{lccc}
\hline
\textbf{Dataset} & \textbf{GNN}   & \textbf{GLNN}  & \textbf{PGKD}  \\ \hline
Cora                         & -0.94 & -0.88 & -0.92 \\
Citeseer                     & -0.71 & -0.62 & -0.67     \\
A-computer                   & -0.75 & -0.60 & -0.77    \\
\hline
\end{tabular}
}
\end{minipage}

\end{table}


==> tables/main_res_wmlp.tex <==
\begin{table}[ht]
\centering
%\tableindent 
\renewcommand\arraystretch{1.2}
\caption{
Experiment results of PGKD on several benchmarks under \textit{transductive} and \textit{inductive} settings.
We report the average test accuracy (\%) and the standard deviation over five runs for each dataset.
% We also report the p-value.
PGKD outperforms GLNN with higher average scores and lower standard deviations.
In particular, for large datasets (Arxiv and Twitch-gamer) with more than 160,000 nodes, PGKD statistically significantly~(p-value < 0.05) outperforms GLNN. 
}
\vspace{0.2cm}
\resizebox{0.9\textwidth}{!}
{%
\begin{tabular}{llllllll}
\hline
\textbf{Dataset}                       & \textbf{GNN Setting} & \textbf{GNN}    & \multicolumn{1}{l}{\textbf{GLNN}}  & \multicolumn{1}{l}{\textbf{MLP}}     & \multicolumn{1}{l}{\textbf{PGKD}~(Ours)}   & \multicolumn{1}{l}{$\Delta$\textbf{GLNN}} \\ \hline
\multirow{2}{*}{Cora}         &  \textit{transductive}  & \multicolumn{1}{l}{81.11$\pm$2.05} & \multicolumn{1}{l}{80.22$\pm$1.81} & \multicolumn{1}{l}{58.89$\pm$2.27} & \multicolumn{1}{l}{82.15$\pm$0.19} & \textbf{$\uparrow$ 1.93}  \\
& \textit{inductive}   & \multicolumn{1}{l}{81.59$\pm$1.95} & \multicolumn{1}{l}{74.38$\pm$0.85} & \multicolumn{1}{l}{57.75$\pm$2.19} & \multicolumn{1}{l}{74.85$\pm$0.24} & \textbf{$\uparrow$ 0.47} \\ \hline
\multirow{2}{*}{Citeseer}     &  \textit{transductive}  & 70.62$\pm$1.53                     & 71.87$\pm$1.90  
& 61.62$\pm$3.99 & 72.93$\pm$1.17 & \textbf{$\uparrow$ 1.06  }                  \\
&  \textit{inductive}   & 69.89$\pm$2.80                     & 69.34$\pm$2.10   & 58.78$\pm$3.97                  & 69.94$\pm$2.03   & \textbf{$\uparrow$ 0.60}                \\ \hline
\multirow{2}{*}{A-computer}   & \textit{transductive}  & 82.70$\pm$0.69                     & 82.84$\pm$1.04  & 63.56$\pm$2.64                   & 83.42$\pm$0.39 & \textbf{$\uparrow$ 0.58   }                \\
& \textit{inductive}   & 83.12$\pm$0.88                    & 80.94$\pm$0.83    & 66.49$\pm$3.06                  & 81.78$\pm$0.50       & \textbf{$\uparrow$ 0.84}              \\ \hline
\multirow{2}{*}{Penn94}       &  \textit{transductive}  & 82.08$\pm$0.40                     & 81.08$\pm$0.50   & 74.01$\pm$0.56                  & 81.51$\pm$0.48  & \textbf{$\uparrow$ 0.43}                   \\
& \textit{inductive}   & 81.95$\pm$0.52                     & 71.67$\pm$0.52  & 74.58$\pm$1.06                   & 72.18$\pm$0.50         & \textbf{$\uparrow$ 0.51}            \\ \hline
\multirow{2}{*}{Arxiv}       & \textit{transductive}  & 70.92$\pm$0.34                     & 63.46$\pm$0.46      & 65.05$\pm$0.49                 & 64.84$\pm$0.25 & \textbf{$\uparrow$ 1.38}                  \\
& \textit{inductive}   & 71.00$\pm$0.28                      & 59.50$\pm$0.34        & 59.50$\pm$0.34              & 59.97$\pm$0.44           & \textbf{$\uparrow$ 0.47}        \\ \hline
\multirow{2}{*}{Pubmed}       & \textit{transductive}  & 76.44$\pm$2.44                     & 76.66$\pm$3.34   & 31.86$\pm$9.10                  & 77.02$\pm$2.85 & \textbf{$\uparrow$ 0.36}                    \\
& \textit{inductive}   & 75.68$\pm$2.80                      & 73.95$\pm$5.56       & 39.83$\pm$2.56              & 76.35$\pm$2.21           & \textbf{$\uparrow$ 1.86 }         \\ \hline
\multirow{2}{*}{Twitch-gamer} &  \textit{transductive}  & 62.58$\pm$0.19                     & 60.07$\pm$0.16     & 60.61$\pm$0.23                & 60.56$\pm$0.07            & \textbf{$\uparrow$ 0.49 }        \\
& \textit{inductive}   & 62.34$\pm$0.44                     & 59.57$\pm$0.30     & 60.26$\pm$0.30                 & 60.01$\pm$0.42      & \textbf{$\uparrow$ 0.44  }             \\ \hline
\end{tabular}
}

\label{tab: main_res}
\end{table}
